Understanding Road Layout from Videos as a Whole

In this paper, we address the problem of inferring the layout of complex road scenes from video sequences. To this end, we formulate it as a top-view road attributes prediction problem and our goal is to predict these attributes for each frame both accurately and consistently. In contrast to prior work, we exploit the following three novel aspects: leveraging camera motions in videos, including context cuesand incorporating long-term video information. Specifically, we introduce a model that aims to enforce prediction consistency in videos. Our model consists of one LSTM and one Feature Transform Module (FTM). The former implicitly incorporates the consistency constraint with its hidden states, and the latter explicitly takes the camera motion into consideration when aggregating information along videos. Moreover, we propose to incorporate context information by introducing road participants, e.g. objects, into our model. When the entire video sequence is available, our model is also able to encode both local and global cues, e.g. information from both past and future frames. Experiments on two data sets show that: (1) Incorporating either globalor contextual cues improves the prediction accuracy and leveraging both gives the best performance. (2) Introducing the LSTM and FTM modules improves the prediction consistency in videos. (3) The proposed method outperforms the SOTA by a large margin.

==> Understanding Road Layout from Videos as a Whole (1)/custom_cmds.tex <==
% This file defines some common commands we'll use during writing.
% requires:
% \usepackage{color}
% \usepackage{ifthen}

% writing helpers
\newcommand{\todo}[1]{{\textcolor{red}{TODO: #1}}}
\newcommand{\sam}[1]{{\textcolor{blue}{SAM: #1}}}
\newcommand{\buyu}[1]{{\textcolor{blue}{BUYU: #1}}}
\newcommand{\bing}[1]{{\textcolor{blue}{BING: #1}}}
\newcommand{\pan}[1]{{\textcolor{blue}{PAN: #1}}}
\newcommand{\manu}[1]{{\textcolor{blue}{MANMOHAN: #1}}}
\newcommand{\rebut}[1]{{\textcolor{blue}{REBUT: #1}}}

% abbrevs
%\newcommand{\eg}{e.g.\@}
%\newcommand{\etal}{et al.\@}
%\newcommand{\etc}{etc.\xspace}
%\newcommand{\ie}{i.e.\@}
%\newcommand{\cf}{cf.\@}
%\newcommand{\wrt}{wrt.\xspace}


% colors
%\definecolor{tablehlcolor}{rgb}{0.6,0.95,0.6}
%\definecolor{tablehlcolor2}{rgb}{0.6,0.6,0.95}
%\definecolor{tablehlcolor3}{rgb}{0.95,0.6,0.6}
%\definecolor{tablehlcolorSolid}{rgb}{0,1,0}
%\definecolor{tablehlcolorSolid2}{rgb}{0,0,1}
%\definecolor{tablehlcolorSolid3}{rgb}{1,0,0}

% figures
\newlength\tikzfigwidth
\newlength\tikzfigheight



==> Understanding Road Layout from Videos as a Whole (1)/notation.tex <==
% This file defines the notation for this project

\def\txtBin{\textrm{b}}
\def\txtMc{\textrm{m}}
\def\txtReg{\textrm{c}}

% The scene attributes
\def\sa{\Theta}
\def\saBin{\sa_{\txtBin}}
\def\saMc{\sa_{\txtMc}}
\def\saReg{\sa_{\txtReg}}
\def\saBinIdx{\sa_{\txtBin{},i}}
\def\saMcIdx{\sa_{\txtMc,i}}
\def\saRegIdx{\sa_{\txtReg,i}}
\def\saBinNum{M^{\txtBin}}
\def\saMcNum{M^{\txtMc}}
\def\saRegNum{M^{\txtReg}}
\def\numSaRegBins{K}
\def\saSim{\sa^{\textrm{s}}}
\def\saReal{\sa^{\textrm{r}}}
\def\saBinRealSim{\saBin}
\def\saMcRealSim{\saMc}
\def\saRegRealSim{\saReg}
\def\saBinRealIdx{\saBinIdx}
\def\saMcRealIdx{\saMcIdx}
\def\saRegRealIdx{\saRegIdx}


% Data
\def\dsReal{D^{\textrm{r}}}
\def\dsSim{D^{\textrm{s}}}
\def\dsRealSize{N^{\textrm{r}}}
\def\dsSimSize{N^{\textrm{s}}}
\def\dsRealSimSize{N^{\{\textrm{r,s}\}}}


% The BEV-maps
\def\bevmap{\mat{x}}
\def\bevmapH{H}
\def\bevmapW{W}
\def\bevmapC{C}
\def\bevmapFeat{f_{\bevmap}}
\def\bevmapFeatDim{D}
\def\bevmapReal{\bevmap^{\textrm{r}}}
\def\bevmapSim{\bevmap^{\textrm{s}}}
\def\bevmapRealSim{\bevmap^{\textrm{r,s}}}
\def\bevmapFeatReal{f_{\bevmapReal}}
\def\bevmapFeatSim{f_{\bevmapSim}}
\def\bevmapFeatRealSim{f_{\bevmapRealSim}}

% Image space
\def\im{\mat{I}}

% Networks and parameters
\def\nnFull{f}
\def\nnFeat{g}
\def\nnFeatReal{g_{\textrm{r}}}
\def\nnFeatSim{g_{\textrm{s}}}
\def\nnAttr{h}
\def\nnFullWgts{\gamma_{\nnFull}}
\def\nnFeatWgts{\gamma_{\nnFeat}}
\def\nnFeatWgtsReal{\gamma_{\nnFeat}^{\textrm{r}}}
\def\nnFeatWgtsSim{\gamma_{\nnFeat}^{\textrm{s}}}
%\def\nnAttrWgts{\gamma_{\nnAttr}}
\def\nnDiscr{d}
\def\nnDiscrWgts{\gamma_{\nnDiscr}}

% Predictions
\def\predSa{\eta}
\def\predSaBin{\predSa_{\txtBin}}
\def\predSaMc{\predSa_{\txtMc}}
\def\predSaReg{\predSa_{\txtReg}}
\def\predSaBinIdx{\predSa_{\txtBin,i}}
\def\predSaMcIdx{\predSa_{\txtMc,i}}
\def\predSaRegIdx{\predSa_{\txtReg,i}}
\def\predSaBinReal{\predSaBin}
\def\predSaMcReal{\predSaMc}
\def\predSaRegReal{\predSaReg}
\def\predSaBinRealIdx{\predSaBinIdx}
\def\predSaMcRealIdx{\predSaMcIdx}
\def\predSaRegRealIdx{\predSaRegIdx}



% Obsolete ...
%\def\paramAttrPred{\gamma_{\textrm{A}}}
%\def\paramBevRefine{\gamma_{\textrm{B}}}
%\def\paramSt{\gamma_{\textrm{C}}}


% Losses
\def\lossSym{\mathcal{L}} % FIXME: This is generic and should be put somewhere else ...

\def\lossSup{\lossSym_{\textrm{sup}}}
\def\lossSupReal{\lossSup^{\textrm{r}}}
\def\lossSupSim{\lossSup^{\textrm{s}}}
\def\lossSupRealSim{\lossSup^{\{\textrm{r,s}\}}}
\def\lossAdv{\lossSym_{\textrm{adv}}}

\def\lossWgtReal{\lambda^{\textrm{r}}}
\def\lossWgtSim{\lambda^{\textrm{s}}}
\def\lossWgtAdv{\lambda^{\textrm{adv}}}

\def\lossBCE{\textrm{BCE}}
\def\lossCE{\textrm{CE}}
\def\lossEllOne{\ell_1}

% Obsolete ...
%\def\lossSaReal{\lossSym_{\textrm{SaReal}}}
%\def\lossSaRealBin{\lossSym_{\textrm{SaReal-Bin}}}
%\def\lossSaRealMc{\lossSym_{\textrm{SaReal-Mc}}}
%\def\lossSaRealReg{\lossSym_{\textrm{SaReal-Reg}}}
%\def\lossDaBevRefine{\lossSym_{\textrm{BevRef}}}
%def\lossDaBevRefineAdv{\lossSym_{\textrm{BevRef-Adv}}}
%\def\lossDaBevRefineRec{\lossSym_{\textrm{BevRef-Rec}}}
%def\lossSaSim{\lossSym_{\textrm{SaSim}}}
%\def\lossDaStyleTranAdv{\lossSym_{\textrm{St-Adv}}}


% General
\def\numTrainSamples{N}







% Network flow - LP
\def\flow{\vec{x}}
\def\flowIn{x^{\textrm{in}}}
\def\flowOut{x^{\textrm{out}}}
\def\flowDet{x^{\textrm{det}}}
\def\flowLink{x^{\textrm{link}}}
\def\flowOpt{\flow^*}
\def\flowGt{\flow^{\textrm{gt}}}

\def\cost{\vec{c}}
\def\costIn{c^{\textrm{in}}}
\def\costOut{c^{\textrm{out}}}
\def\costDet{c^{\textrm{det}}}
\def\costLink{c^{\textrm{link}}}

\def\costUnary{\vec{c}^{\textrm{U}}}
\def\costPairwise{c^{\textrm{P}}}

\def\costFin{\vec{f}}
\def\costFpa{\mathbf{\Theta}}

\def\Nvars{M}



% Optimization
\def\opttemp{t}



% Detections
\def\det{\vec{d}} % a detection

\def\bboxIdx{i} % index
\def\bboxIdxAlt{j} % alternative index
\def\bboxN{K} % number of all detections in the graph

\def\bbox{\vec{b}(\det)} % a bounding box, also a detection
\newcommand{\detBox}[1]{\ensuremath{\vec{b}(#1)}}
\def\bboxS{s(\det)} % corresponding detection score or confidence
\def\bboxP{p(\det)} % detection probability
\newcommand{\detProb}[1]{\ensuremath{p(#1)}}
\def\bboxT{t(\det)}
\newcommand{\detFrame}[1]{\ensuremath{t(#1)}}




% Trajectories
\def\traj{\mathcal{T}}
\def\trajIdx{k}
\def\trajSize{N_\trajIdx}
\def\trajSingle{\mathtt{t}}



% Tracker
\def\winsize{W}





% math
\def\realspace{\mathbb{R}} % the real space
\def\intspace{\mathbb{Z}} % the integer space

\newcommand{\mat}[1]{\ensuremath{\mathbf{#1}}}
\let\Oldvec\vec \renewcommand{\vec}[1]{\ensuremath{\mathbf{#1}}}
\def\transp{\top} % transpose sign; alternative: \textrm{T}

\newcommand{\intd}[1]{{\rm d}#1} % the d in the integral
\newcommand{\dotp}[2]{<#1,#2>} % dot product
\newcommand{\eye}{\mat{I}} % identity matrix
\newcommand{\pderi}[2]{\ensuremath{\frac{\partial #1}{\partial #2}}} % partial derivative
\newcommand{\deri}[2]{\ensuremath{\frac{{\rm d}#1}{{\rm d}#2}}} % partial derivative
\newcommand{\dirac}{\ensuremath{\delta}} % dirac delta function
\newcommand{\conv}{\ensuremath{\ast}} % convolution
\def\abs#1{\left| #1 \right|}
\def\norm#1{\left|\left| #1 \right|\right|}

\newcommand{\nullspace}[1]{\ensuremath{\mathcal{N}\left(#1\right)}} % null space

\def\sgn{\mathop{\rm sgn}} % signum
\def\cos{\mathop{\rm cos}} % cos
\def\sin{\mathop{\rm sin}} % sin
%\DeclareMathOperator*{\argmin}{arg\,min} % argmin
%\DeclareMathOperator*{\argmax}{arg\,max} % argmax
\newcommand{\trace}[1]{\mbox{tr}\left( #1 \right)} % trace of a matrix
\renewcommand{\det}[1]{\mbox{det}\left( #1 \right)} % trace of a matrix

\newcommand{\N}[3][]{\ensuremath{\mathcal{N}^{#1}(#2,#3)}} % normal distribution
\newcommand{\chis}[2][non]{\ensuremath{\chi^2 \ifthenelse{\equal{#1}{non}}{}{ \left(#1,#2\right)}}} % Chi^2 distribution
\newcommand{\Gammaf}[1][non]{\ensuremath{\Gamma\ifthenelse{\equal{#1}{non}}{}{ \left( #1 \right)}}} % gamma distribution
\def\normdistr{\mathcal{N}} % normal distribution
\newcommand{\unifdiscrdistr}[2]{\ensuremath{\mathcal{U}\{#1,#2\}}} % discrete uniform distribution
\newcommand{\unifcontidistr}[2]{\ensuremath{\mathcal{U}(#1,#2)}} % continuous uniform distribution
\newcommand{\condprob}[2]{\ensuremath{p(#1|#2)}} % conditional probability
\newcommand{\condprobsub}[3]{\ensuremath{p_{#3}(#1|#2)}} % conditional probability (with some subscript)
\newcommand{\E}[1]{\ensuremath{\textrm{\textbf{E}}\left[#1\right]}} % expectation operator
\newcommand{\Esub}[2]{\ensuremath{\textrm{\textbf{E}}_{#1}\left[#2\right]}} % expectation operator with subscript
\newcommand{\std}[1]{\ensuremath{\textrm{std} (#1) }} % standard deviation

\def\mm{\hspace{-1.5mm}\rule[1mm]{1.3mm}{0.15mm}\rule{0.2mm}{0mm}\relax}    % short minus symbol


\newcommand{\degree}[1][non]{\ensuremath{\ifthenelse{\equal{#1}{non}}{^\circ}{#1^\circ}}} % degree
% makes all sqrts closed
\LetLtxMacro{\oldsqrt}{\sqrt}
\renewcommand{\sqrt}[1][\ ]{%
  \def\DHLindex{#1}\mathpalette\DHLhksqrt}
\def\DHLhksqrt#1#2{%
  \setbox0=\hbox{$#1\oldsqrt[\DHLindex]{#2\,}$}\dimen0=\ht0
  \advance\dimen0-0.2\ht0
  \setbox2=\hbox{\vrule height\ht0 depth -\dimen0}%
  {\box0\lower0.71pt\box2}}
\def\covarmat{\mat{\Sigma}} % covariance matrix
\newcommand{\indicator}[1]{\ensuremath{\mathbbm{I}\left[#1\right]}} % indicator function
\newcommand{\cardinality}[1]{\ensuremath{\left|#1\right|}} % cardinality of a set


%\newcommand{\loss}[1]{\ensuremath{\mathcal{L}\left(#1\right)}} % loss function
%\def\lossSym{\mathcal{L}}

% +++ DATA ***
%\def\dataspace{\mathcal{X}}
%\def\labelspace{\mathcal{Y}}
%\def\datadim{\mathtt{D}}
%\def\outdim{\mathtt{K}}
%\def\nclasses{\mathtt{C}}
%\def\ci{\mathtt{c}}
%
%\def\dataset{\vec{X}} % it was \vec{D}
%\def\datasetD{\dataset_{\dataspace}}
%\def\datasetL{\dataset_{\labelspace}}
%\def\ndata{\mathtt{N}}
%\def\di{\mathtt{n}} % data sample index
%\def\bag{\vec{B}}
%
%\def\dsample{\vec{x}}
%\def\dlabel{\vec{y}}
%\def\dweight{w}
%\def\dgrad{\vec{g}}
%\def\dresidual{\vec{r}}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "param_bev"
%%% End:


==> Understanding Road Layout from Videos as a Whole (1)/sections/abstract.tex <==
\begin{abstract}
%V3
In this paper, we address the problem of inferring the layout of complex road scenes from video sequences. To this end, we formulate it as a top-view road attributes prediction problem and our goal is to predict these attributes for each frame both accurately and consistently. In contrast to prior work, we exploit the following three novel aspects: leveraging camera motions in videos, including context cues and incorporating long-term video information. Specifically, we introduce a model that aims to enforce prediction consistency in videos. Our model consists of one LSTM and one Feature Transform Module (FTM). The former implicitly incorporates the consistency constraint with its hidden states, and the latter explicitly takes the camera motion into consideration when aggregating information along videos. Moreover, we propose to incorporate context information by introducing road participants, e.g. objects, into our model. When the entire video sequence is available, our model is also able to encode both local and global cues, e.g. information from both past and future frames. Experiments on two data sets show that: (1) Incorporating either global or contextual cues improves the prediction accuracy and leveraging both gives the best performance. (2) Introducing the LSTM and FTM modules improves the prediction consistency in videos. (3) The proposed method outperforms the SOTA by a large margin.

% we firstly map the perspective image to a semantic top-view representation. To achieve that, we propose to consider both local and global, e.g. information in past and future frames, cues. Moreover, we also incorporate context information by introducing road participants, e.g. objects, in our top-view representation. Then we propose a model that aims to enforce prediction consistency in videos. Our model consists of a LSTM as well as a Feature Transform Module (FTM). The former implicitly incorporates the consistent constraints with its hidden states, and the later explicitly takes the camera motion into consideration when aggregating information along videos. Experiments in two data sets show that: (1) Incorporating either global or context cues improves the prediction accuracy and the one that leveraging both gives the best performance. (2) Our LSTM, as well as the FTM, can further improve the prediction consistency in videos. (3) Our proposed method outperforms the SOTA by a large margin.

%V2
%In this paper, we address the problem of inferring the layout of complex road scenes from video sequences. To this end, we formulate it as a top-view road attribute prediction problem and our goal is to predict the road layout for each frame both accurately and consistently. In contrast to prior work, we exploit the following three novel aspects, incorporating long-term video information, including context cues as well as leveraging camera motions in videos. Specifically, we firstly map the perspective image to a semantic top-view representation. To achieve that, we propose to consider both local and global, e.g. information in past and future frames, cues. Moreover, we also incorporate context information by introducing road participants, e.g. objects, in our top-view representation. Then we propose a model that aims to enforce prediction consistency in videos. Our model consists of a LSTM as well as a Feature Transform Module (FTM). The former implicitly incorporates the consistent constraints with its hidden states, and the later explicitly takes the camera motion into consideration when aggregating information along videos. Experiments in two data sets show that: (1) Incorporating either global or context cues improves the prediction accuracy and the one that leveraging both gives the best performance. (2) Our LSTM, as well as the FTM, can further improve the prediction consistency in videos. (3) Our proposed method outperforms the SOTA by a large margin.

% V1
%In this paper, we address the problem of inferring the layout of complex road scenes given video sequences as input. Specifically, we firstly obtain a semantic map in top-view. Our top-view map considers cues both from individual frame and entire/global video sequence thus is more accurate and temporally coherent. Moreover, we further demonstrate the effectiveness of incorporating context information by introducing road participants in top-view maps. Given the top-view map as input, we then train a deep neural network to infer the scene model's parameters w.r.t. pre-defined layout attributes. To further enforce the temporal consistency in video predictions, we introduce LSTM and Spatial Transform Module (STM) in our network. The LSTM module implicitly incorporates the consistent constraints with its hidden status. And the STM module takes the camera motion into consideration and enforces the temporal smoothness in predictions by aggregating features between consecutive frames in video sequences. Experiments in two data sets show that: (1) Our proposed top-view maps that include individual frame, global video sequences and context information can improve the prediction accuracy of layout estimation task (2) Our LSTM, as well as the STM, can further improve the temporally consistency in video sequences.

% V3
% In this paper, we address the problem of inferring the layout of complex road scenes given a single camera as input.  To achieve that, we first propose a novel parameterized  model of road layouts in a top-view representation, which is not only intuitive for human visualization but also provides an interpretable interface for higher-level decision making.  Moreover, the design of our top-view scene model allows for efficient sampling and thus generation of large-scale simulated data, which we leverage to train a deep neural network to infer our scene model's parameters.  Specifically, our proposed training procedure uses supervised domain-adaptation techniques to incorporate both simulated as well as manually annotated data.  Finally, we design a Conditional Random Field (CRF) that enforces coherent predictions for a single frame and encourages temporal smoothness among video frames.  Experiments on two public data sets show that: (1) Our parametric top-view model is representative enough to describe complex road scenes; (2) The proposed method outperforms baselines trained on manually-annotated or simulated data only, thus getting the best of both; (3) Our CRF is able to generate temporally smoothed while semantically meaningful results.

\end{abstract}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../param_bev"
%%% End:


==> Understanding Road Layout from Videos as a Whole (1)/sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
In this work, we present a scene understanding framework to estimate the parametric road layout in each view in a video. In constrast to the case with only single image input, we propose to make use of the temporal information in videos by leveraging LSTM/FTM model, context information as well as global 3D reconstruction, altogether leading to very promising results.  
%inputs the video sequences and outputs the road layout. 

%Compared to existing work, our main contributions that: (1) we demonstrate the effectiveness of combining local and global information in videos. We also show that our layout estimation task benefits from context information. (2) we propose to utilize Feature Transform Module (FTM) to aggregate the information in top-view from past frames w.r.t. camera motions to explicitly encourage prediction coherency. More importantly, we introduce LSTM to further improve the prediction in consecutive frames. Experiments on two data sets show that: (1) Incorporating global and context information can boost the prediction accuracy individually and combining them together can give us the best performance. (2) Given video sequence as input, LSTM and FTM can further boost the prediction accuracy as well as the temporal smoothness. 

%In this work, we present a scene understanding framework for complex road scenarios. Our key contributions are:  (1) A parameterized and interpretable model of the scene that is defined in the top-view and enables efficient sampling of diverse scenes.  The semantic top-view representation makes rendering easy (compared to photo-realistic RGB images in perspective view), which enables the generation of large-scale simulated data.  (2) A neural network design and corresponding training scheme to leverage both simulated as well as manually-annotated real data.  (3) A graphical model that ensures coherent predictions for a single frame input and temporally smooth outputs for a video input.
%Our proposed hybrid model (using both sources of data) outperforms its counterparts that use only one source of supervision in an empirical evaluation. This confirms the benefits of the top-view representation, enabling simple generation of large-scale simulated data and consequently our hybrid training.

% \paragraph{Acknowledgements:} We want to thank Kihyuk Sohn for valuable discussions on domain adaptation and all anonymous reviewers for their comments.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../param_bev"
%%% End:


==> Understanding Road Layout from Videos as a Whole (1)/sections/experiments.tex <==
\section{Experiments}
\label{sec:exps}


%In this section, we demonstrate the effectiveness of our proposed method by conducting several experiments on two data sets and analyzing the importance of different components of our model.
%Specifically, we compare with several baselines and demonstrate our key contributions: 1) improving the single image prediction accuracy with the use of global and context information 2) enforcing temporal smoothness in videos with the help of FTM and LSTM. 

In this section, we demonstrate the effectiveness of our proposed augmented input representation and LSTM/FTM by conducting several experiments on two data sets. 

\paragraph{Datasets:}
We validate our ideas on two data sets, KITTI~\cite{sam:Geiger13a} and NuScenes~\cite{sam:NuScenes18a}. Similarly, we utilize the annotated data in~\cite{Wang_2019_CVPR}, which includes around 17000 annotations for KITTI~\cite{sam:Geiger13a} and about 1200 annotations %\footnote{Note that in the original paper~\cite{Wang_2019_CVPR}, they utilize around 3000 images in total and the ratio between training and testing is about 3 to 1. However, in our setting, we have 1165 images for training and 348 for testing. So the results are not directly comparable. The main difference between our setting and theirs is that we remove sequences where cars are not moving at all.} 
for NuScenes~\cite{sam:NuScenes18a} in terms of scene layout annotation. To train our segmentation network, we further have 1243 images for training and 382 for testing on KITTI. We refer the readers to~\cite{Wang_2019_CVPR,Wang_2019_CVPRworkshop} for more details of data sets and implementation details can be found in supplementary. %\sam{We could cite the workshop paper for the dataset too.}

\begin{table}\centering\small
\setlength{\belowcaptionskip}{-0.4cm}
  \input{tables/nuscene_results.tex}
  \vspace{-0.2cm}
  \caption{Results on road scene layout estimation on~\cite{sam:NuScenes18a}. %Note that we use far less real annotations compared to~\cite{Wang_2019_CVPR} and we do not utilize simulated data.
  }
  \label{tbl:sub_exp_layout}
\end{table}

\begin{figure*}%{\textwidth}
    \setlength{\abovecaptionskip}{-0.0cm}    
    \setlength{\belowcaptionskip}{-0.4cm}
    \vspace{-0.2cm}
    \begin{minipage}[h]{0.6\textwidth}
        \centering
        \input{tables/main_exp_layout}
        \makeatletter\def\@captype{table}\makeatother\caption{Main results on road scene layout estimation on KITTI~\cite{sam:Geiger13a}. We can see that: 1) The global (BEV-C, BEV-J) and context (BEV-J-O) information do benefits the single image performance compared to their single image competitors. 2) Introducing LSTM and FTM can further improve the accuracy compared to single image method.}
        \label{tbl:main_exp_layout}
    \end{minipage}
    \hspace{0.2cm}
    \begin{minipage}[h]{0.38\textwidth}
        \centering
        \setlength{\abovecaptionskip}{-0.2cm}    
        \includegraphics[height=0.4\textwidth, trim = 0mm 140mm 170mm 10mm, clip]{figures/teaser.pdf}
        \includegraphics[height=0.4\textwidth, trim = 90mm 140mm 68mm 10mm,clip]{figures/teaser.pdf}
        \makeatletter\def\@captype{figure}\makeatother\caption{Illustrations of baseline model architectures. We denote the upper one as $basic$ and lower one as $blstm$.}
        \label{fig:archs_overview}  
    \end{minipage}
\end{figure*}
  
  
\paragraph{Evaluation metrics:}
Since our output space consists of three types of predictions and involves both discrete and continuous variables, we follow the metrics defined in~\cite{Wang_2019_CVPR} and summarize them below.

As for binary variables $\saBin$ (like the existence of crosswalk on the main road or left side-walk) and for multi-class variables $\saMc$ (like the number of lanes on your left), we report the prediction accuracy as $\textrm{Accu.-Bi} = \frac{1}{14} \sum_{k=1}^{14} [p_k = \saBin{}_k]$ and $\textrm{Accu.-Mc} = \frac{1}{2} \sum_{k=1}^{2} [p_k = \saMc{}_k]$. More importantly, since we observe that the binary classes are extremely biased, we also report the F1 score on $\saBin$ which better informs the overall performance. Specifically, $\textrm{F1.-Bi} = \frac{1}{14} \sum_{k=1}^{14} 2 \times \frac{p_k \times r_k}{p_k + r_k}$, where $p_k$ and $r_k$ are the precision and recall rate on $k$-th variable of binary attributes.
For regression variables we use the mean square error (MSE).  

In addition, we also report Intersection-over-Union (IoU) as a overall performance evaluation metric. Specifically, we assume that we can render four-class semantic top-view maps with either the predicted results or the ground-truth annotations. Then we report the average IoU score over all test images. More details on IoU are presented in supplementary.%Note that compared to traditional IoU score in semantic segmentation task, our IoU is different in the a few aspects (discussed in supplementary material).

%: 1) the semantic top-view maps from predicted results are obtained with some rendering functions, which are highly nonlinear and cannot be directly optimized 2) the rendered semantic top-view maps entangle all three types of attributes together and their impacts on IoU varies a lot. For instance, predicting the number of lanes on the left incorrectly by one has a bigger impact than getting the distance to a crosswalk wrong by one meter. 


% \begin{figure*}\centering
% \includegraphics[width=1.0\textwidth]{figures/model_archs_boxes.png}
% \vspace{-0.65cm}
% \caption{Illustrations of all the models we compare in the quantitative evaluation in Tab.~\ref{tbl:main_exp_layout}.\buyu{To be updated}}
% \label{fig:archs_overview}
% \end{figure*}

\iffalse
\begin{figure*}[t]

    \begin{center}
        \includegraphics[width=0.8\linewidth, trim = 0mm 140mm 60mm 10mm, clip]{figures/models.pdf}
    \end{center}
    \vspace{-0.85cm}
    \caption{Illustrations of baseline model architectures. We denote the upper one as $basic$ and lower one as $b-LSTM$.}
    \label{fig:archs_overview}
\end{figure*}
\begin{table*}\centering\small
  \input{tables/main_exp_layout}
  \vspace{-0.2cm}
  \caption{Main results on road scene layout estimation on KITTI~\cite{sam:Geiger13a}. We can see that: 1) The global (BEV-C, BEV-J) and context (BEV-J-O) information do benefits the single image performance compared to their single image competitors. 2) Introducing LSTM and FTM can further improve the accuracy compared to single image method.~\buyu{Note that top two performances are bold in this table.}}
  \label{tbl:main_exp_layout}
\end{table*}
\fi


\subsection{Evaluations on Global and Context Cues}
In this section, we would like to explore the impact of $bev\text{-}final$. To this end, we aim to validate the effectiveness of our proposed context and global information on road layout prediction. We use the basic model without LSTM and FTM, unless otherwise specified. Details for this basic model can be found in $basic$ of Fig.~\ref{fig:archs_overview}. %and shall add LSTM later. Details for these two models are visualized in $basic$ and $blstm$ in Fig.~\ref{fig:archs_overview} respectively.

\paragraph{Baselines:}
We compare our proposed method with several competing methods presented in~\cite{Wang_2019_CVPR}. The~\textbf{RGB} method takes a single perspective RGB image as input and trains a model~\cite{sam:He16a} that directly outputs predictions for scene attributes. The~\textbf{RGB+D} method shares the same model architecture w.r.t.~\textbf{RGB} but outputs both per-pixel depth map and attribute predictions. Both~\textbf{BEV} and the SOTA~\textbf{H-BEV-DA} output scene attributes with $bev$ as input, which means they are all online methods. The differences lie in: 1) the former uses only $bev$ from real images during training while the latter utilizes additional simulated $bev$; 2) the former uses $basic$ model and the later has a hybrid model as in~\cite{Wang_2019_CVPR}. Note that +GM means a spatial-temporal graphical model is added as post-processing.

% and then also include the last one as the direct baseline to study the impact of our augmented input representation. 
%
% \begin{itemize}
% \item \textbf{RGB (RGB):} A ResNet-101~\cite{sam:He16a} trained on the manually-annotated ground truth and predicts all attributes simultaneously in a multi-task setup.
% \item \textbf{RGB+Depth (RGB+D):} We introduce another task, or pixel-level depth prediction task, in RGB model. %Intuitively, such additional task would benefit the regression task, \eg , distance to the crosswalk. More importantly, the M-RGB+D model unitizes the same information as M-BEV as introduced below. 
% \item \textbf{Hybrid-GT-BEV (H-BEV-DA):} This is the previous SOTA as suggested by~\cite{Wang_2019_CVPR}. In this case, both simulated and real data are exploited and domain transform is introduced to bridge the gap between these two. Note that +GM means we add spatial-temporal graphical model as post-processing.
% \item \textbf{BEV (BEV):} This is our direct baseline to compare with. We feed $bevinit$ obtained locally with individual frame into the model shown in the upper figure of Fig.~\ref{fig:archs_overview}. Again, +GM means we include spatial-temporal graphical model in this model.
% \end{itemize}

\paragraph{Our proposals:}
Apart from baselines, we further propose the following methods with different input representations:
%

\begin{itemize}
\item \textbf{BEV-COLMAP (BEV-C):} %Instead of replying the semantic and depth prediction from one frame to get the four-class top-view maps, we turn to 3D point clouds obtained from the entire video sequence for better quality 
We propose $bev$-$col$ with global information from videos, as described in Sec.~\ref{sec:input_ind_and_colmap}. Once we get the $bev$-$col$, we feed it to the $basic$ model. 
%We refer the readers to the second paragraph in Sec.~\ref{sec:input_ind_and_colmap} for more details.
\item \textbf{BEV-JOINT (BEV-J):} We combine the $bev$ and $bev$-$col$ together and obtain the input for BEV-J. Then we feed the joint input to the $basic$ model.
\item \textbf{BEV-JOINT-OBJ (BEV-J-O):} As described in Sec.~\ref{sec:context}, we further add object information and obtain $bev$-$final$ as the input for BEV-J-O. Again, a $basic$ model is learned.
\end{itemize}

\paragraph{Quantitative results:}
Tab.~\ref{tbl:main_exp_layout} summarizes our main results on KITTI~\cite{sam:Geiger13a}. We have the following observations. Firstly,  comparing BEV-C to BEV, we can see that obtaining global information from 3D point clouds generated with the entire video sequence is better than relying on individual depth and semantic segmentation results, e.g. large improvement in F1 score. This improvement might come from higher quality of $bevinit$, especially in terms of both higher accuracy in regions that are far away from the camera and more consistent results. Second, if we compare BEV-J to BEV-C and BEV, we can see that combining them together can further boost the performance for all attributes, e.g. $1.4\%$, $3.3\%$ and $0.04$ improvement for binary, multiclass and regression tasks. More importantly, we can improve the IoU by around $10\%$. One reason might be that the input from BEV-C focuses more on texture regions that can be both close by and far away while input from BEV keeps more details for all close by regions. They are mutual beneficial in terms of representing scene layout in top-view. Finally, once adding object information (BEV-J-O), we can further boost the F1 score by about $5\%$. In conclusion, we can observe a clear improvement when adding individual components. 

We also report partial results on NuScenes~\cite{sam:NuScenes18a} in Tab.~\ref{tbl:sub_exp_layout} and refer the readers to supplementary for complete ones. As for NuScenes~\cite{sam:NuScenes18a}, we again observe that combining individual and global information provides better results than either one in isolation. Also, adding context information further introduces improvements on almost all tasks.
%Results on NuScenes~\cite{sam:NuScenes18a} can be found in Tab.~\ref{tbl:sub_exp_layout}. First, we note that our best model does not outperform \cite{Wang_2019_CVPR}. This is probably due to the small number of training data available in NuScenes such that the synthetic date used in \cite{Wang_2019_CVPR} plays a significant role for superior performance. However, we do observe that our accuracy increases with more augmented input representations.

\paragraph{Ablation study:}
Since the main improvement of the performance boost comes from information of the full video sequence as well as objects, in this section, we conduct ablation studies on: 1) the impact of the quality of top-view maps generated with full video sequences on models, and 2) the impact of the representation of objects on models. Tab.~\ref{tbl:single_ablation_table} summarizes our results, where *-denseC means we change 3D reconstruction parameter of COLMAP to generate much denser $bev$-$col$ as inputs to train our model. And *-C-O means we combine the input from BEV-C with object information and learn to predict the road attributes.

\begin{table}\centering\small
\setlength{\belowcaptionskip}{-0.4cm}
  \input{tables/ablation_single.tex}
  \vspace{-0.2cm}
  \caption{Ablation study on single image based road layout prediction. We abbreviate BEV as $*$ in this table.}
  \label{tbl:single_ablation_table}
\end{table}

\begin{figure*}
    \setlength{\belowcaptionskip}{-0.4cm}
	\centering
	\vspace{-0.4cm}
	\begin{tabular}{ccc}
		\includegraphics[width=0.31\textwidth]{figures/qualit_res/0000000029_new.png} 
		& \includegraphics[width=0.31\textwidth]{figures/qualit_res/0000000631_new.png}
		&\includegraphics[width=0.31\textwidth]{figures/qualit_res/0000000850_new.png} \\
		\includegraphics[width=0.31\textwidth]{figures/qualit_res/0000001207_new.png}
		&\includegraphics[width=0.31\textwidth]{figures/qualit_res/0000001743_new.png} 
		& \includegraphics[width=0.31\textwidth]{figures/qualit_res/0000001887_new.png} \\
	\end{tabular}
	\vspace{-0.35cm}
	\caption{Qualitative results of full model on individual frames from KITTI.  Each example shows perspective RGB, ground truth and predicted semantic top-view (including the object bounding box as green rectangular), respectively.}
	\label{fig:GM_output_more}
\end{figure*}
 
\begin{figure*}
    \setlength{\belowcaptionskip}{-0.4cm}
	\centering
	\begin{tabular}{ccc}
	\includegraphics[width=0.31\textwidth]{figures/qualit_res/0000000356_new.png} 
	& \includegraphics[width=0.31\textwidth]{figures/qualit_res/0000000357_new.png} 
	& \includegraphics[width=0.31\textwidth]{figures/qualit_res/0000000360_new.png} \\
	\includegraphics[width=0.31\textwidth]{figures/qualit_res/0000002046_new.png} 
	& \includegraphics[width=0.31\textwidth]{figures/qualit_res/0000002047_new.png} 
	&\includegraphics[width=0.31\textwidth]{figures/qualit_res/0000002048_new.png} \\
	% Example Seq.1 & Example Seq.2 
	\end{tabular}
	\vspace{-0.35cm}
	\caption{Qualitative results comparing BEV-J-O and full model in \textbf{consecutive} frames of two example sequences from KITTI.  We visualize for each view the perspective RGB image, prediction from BEV-J-O and from full model, respectively.}
	\label{fig:GM_output}
\end{figure*}

As can be seen in this table, denser $bev$-$col$ can definitely improve the performance for all tasks and measurements, which indicates that there can be more room to boost prediction accuracy by improving the quality of $bev$-$col$. Additionally, further performance boosts can be obtained with object information, which again proves that context information can be very useful in our layout prediction task.  



\begin{table}\centering\small
\setlength{\belowcaptionskip}{-0.4cm}
  \input{tables/consistency_check}
  \vspace{-0.3cm}
  \caption{Main results on consistency measurements.}
  \label{tbl:consistency_table}
\end{table}
% \vspace{-0.9cm}




\paragraph{Qualitative results:}
We show several qualitative results in Fig.~\ref{fig:GM_output_more}. We can see from the examples that our model successfully describes a diverse set of road scenes. Moreover, our predictions are generally consistent w.r.t. object detection results.






\subsection{Evaluations on LSTM and FTM}
We further demonstrate the effectiveness of LSTM and FTM in Tab.~\ref{tbl:main_exp_layout}. More specifically, +LSTM model is illustrated in Fig.~\ref{fig:archs_overview} ($blstm$ part) and +LSTM+FTM is our full model. Both models receive $bev$-$final$ as input.

As can be seen in this table, with the help of LSTM, we can increase performance on the binary and regression tasks. Note that we can further boost the F1 score by at least $4\%$ compared to single image methods. More importantly, our full model, or +LSTM+FTM, provides the best overall performance. As highlighted in the table, it almost always performs the best or second best among all tasks and measurements. Even compared to previous SOTA that is trained with both real and simulated data and includes a spatio-temporal graphical model as post-processing, we can clearly observe that the proposed method provides better results, specifically for F1 score. In conclusion, we demonstrate the effectiveness of FTM and LSTM in terms of improving prediction accuracy. We also report the BEV+LSTM in Tab.~\ref{tbl:single_ablation_table}. We can observe that adding LSTM ($blstm$) can improve the performance even with $bev$ inputs, which demonstrates the effectiveness of temporal information on locally obtained top-view representations. Such trend is also shared on NuScenes in Tab.~\ref{tbl:sub_exp_layout}.

\paragraph{Consistency:}
Since we are working in videos, we also analyze the consistency in predictions. To this end, we utilize the following metrics as suggested in~\cite{Wang_2019_CVPR} and refer the readers to supplementary material for more details:

\begin{itemize}
\item {\em Semantic consistency:} we report the average conflicts in attribute predictions. % w.r.t. their semantic meanings. 
% Since no constraints are enforced explicitly in models, it is likely that they output infeasible predictions. %, e.g. one binary variable predicts [no sideroads] but another one predicts [crosswalk on the left side of intersection]. In this case, 
% We count one infeasible prediction 
% \sam{I'm not sure if it is clear to the reader what infeasible means here since we did not explain the graphical model or the scene model} 
% as a conflict. More details can be found in~\cite{Wang_2019_CVPR}.
%Since no constraints are enforced explicitly in models, it is likely that they output infeasible predictions, e.g. one model predicts that there exists no sideroads but has a crosswalk on the left side of intersection. In this case, we count a conflict if the predicted attributes are node feasible and report the average number of conflicts as our semantic consistency measurements.
\item {\em Temporal consistency:} we also report the average number of changes in our prediction. %Specifically, if the prediction for one attribute changes in consecutive frame, we count it as a change. 
% Intuitively, a good model should have lower number in this measurement. Note that we only consider the binary and multiclass tasks in this measurement. Also, since the predictions can be consistently wrong over time, consistency itself cannot replace accuracy.  
\end{itemize}

We show in Tab.~\ref{tbl:consistency_table} quantitative results for the temporal as well as semantic consistency metrics defined on the two data sets. Compared to the single image baseline, we can observe significant improvement from the proposed BEV-J-O in consistency for both data sets. Also, if we compare with video-based existing work, combined with the prediction accuracy shown in Tab.\ref{tbl:main_exp_layout}, we can see that the proposed method outperforms previous SOTA, e.g. boost the accuracy while not sacrificing temporal smoothness. Results and our analysis on NuScenes~\cite{sam:NuScenes18a} can be found in the supplementary.  

Finally, we visualize qualitative results of consecutive frames in two test sequences from KITTI in Fig.~\ref{fig:GM_output}. As can be seen, our model successfully enforces temporal smoothness. We can also observe more consistent predictions, \eg, width of side-road and delimiter width, with the help of the LSTM and FTM. Again, our predictions are consistent w.r.t. object detection results.



%Combined with the prediction accuracy shown in Tab.\ref{tbl:main_exp_layout}, we can see that the proposed method outperforms previous SOTA as well as all baselines.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../param_bev"
%%% End:


==> Understanding Road Layout from Videos as a Whole (1)/sections/intro.tex <==
\section{Introduction}
\label{sec:intro}
Understanding 3D properties of road scenes from single or multiple images is an important and challenging task. Semantic segmentation~\cite{sam:RotaBulo18a,sam:Chen18a,sam:Zhao17a}, (monocular) depth estimation~\cite{sam:Godard17a,sam:Laina16a,sam:Xu18a} and road layout estimation~\cite{sam:Guo12a,sam:Schulter18a,sam:Sengupta12a,Wang_2019_CVPR} are some well-explored directions for single image 3D scene understanding. %which enables many applications like autonomous driving and driver assistance systems generally require understanding for road layouts.
Compared to image-based inputs, videos provide the opportunity to exploit more cues such as temporal coherence, dynamics and context \cite{liu2015multiclass}, yet 3D scene understanding in videos is relatively under-explored, especially with long-term inputs. 
This work takes a step towards 3D road scene understanding in videos through a holistic consideration of local, global and consistency cues.
%In this work, we focus on road scene video understanding and aim to explore multiple aspects in videos as a whole. 
%In this work, we aim to tackle the 3D scene understanding problem in road scene videos.

% Videos provide the opportunity to exploit cues such as temporal coherence, dynamics and context.
% We propose video 3D scene understanding in road scenes.
%Layout understanding in videos is an important while challenging task, e.g., applications like autonomous driving and driver assistance systems generally require understanding for road layouts. %Although road maps could be available with heavy annotations, it is difficult to obtain a world-scale map. %which enables us to perform down-stream applications such as robot navigation, driver assistance systems or autonomous driving. 
%Some works formulate it as a pixel-level semantic segmentation~\cite{sam:RotaBulo18a,sam:Chen18a,sam:Zhao17a} or (monocular) depth estimation~\cite{sam:Godard17a,sam:Laina16a,sam:Xu18a} problem. Others propose to build better representations to reason about occlusions in 3D in either non-parametric~\cite{sam:Guo12a,sam:Schulter18a,sam:Sengupta12a} or parametric~\cite{Wang_2019_CVPR} forms. However, the existing work usually requires heavy additional input data~\cite{sam:Mattyus16a}, unable to work with complex road scenes~\cite{sam:Geiger14a} or not consider multiple aspects of videos~\cite{Wang_2019_CVPR}, e.g. context information or long-term consistency, explicitly. 

%explicitly considers video as input or explores multiple aspects in videos.

%. In this paper, we follow the parametric model proposed in~\ref{Wang_2019_CVPR} that describing complex road layouts in a top-view representation. More specifically, this model describes important scene attributes like the number and width of lanes, and the existence of, and distance to various types of intersections, crosswalks and sidewalks. However, very few of existing work explicitly considers the video as input or tries to enforce temporal smoothness as well as improves the prediction accuracy simultaneously. 

\begin{figure}\centering
  \includegraphics[width=1.09\linewidth, trim = 0mm 30mm 100mm 80mm, clip]{figures/teaser.pdf}
  \vspace{-0.65cm}
  \caption{
  Given perspective images (top left) that captures a 3D scene, our goal is to predict the layout of complex driving scenes in top-view both  accurately and coherently.% (top right). 
  }
  \label{fig:teaser}
\end{figure}

To this end, we formulate this video scene understanding problem as a road layout estimation problem. We are particularly interested in estimating top-view representations~\cite{sam:Schulter18a,sam:Seff16a} as working in the top-view is beneficial for higher-level reasoning and decision making for downstream applications, e.g. path planning and autonomous driving. % as it provides a tangible interface to the real world. 
Given a video sequence, our goal is to predict the road layout of each frame both accurately and coherently. %To start with, we follow the parametric representation proposed in~\cite{Wang_2019_CVPR}. In brief, this road layout representation defines important scene attributes like the number and width of lanes, and the existence of, and distance to various types of intersections, crosswalks and sidewalks in top-view.
%In this work, we focus on understanding road layout from video sequences and propose to explore multiple aspects, e.g. long-term consistency and context, explicitly in videos. To start with, we follow the parametric representation proposed in~\cite{Wang_2019_CVPR}. In brief, this road layout representation defines important scene attributes like the number and width of lanes, and the existence of, and distance to various types of intersections, crosswalks and sidewalks in top-view. Then the authors formulate the road layout estimation task as a scene attributes prediction problem and propose a model that inputs the perspective image and outputs the predicted attributes. Similarly, we propose a model that takes monocular videos in and outputs layout predictions for each frame. In order to make accurate yet consistent predictions in videos, we propose to increase the representation power of model input and enforce prediction consistency in model design by leveraging video as a whole. 

%combine the information locally from individual frame with that globally from entire video sequences. We further incorporate context information, or object information, explicitly.

% In this work, we focus on understanding road layout from videos and propose to utilize information explicitly and implicitly from multiple aspects. Specifically, given a video sequence, our goal is to predict the road layout in each frame in a temporally smooth manner. To this end, we first follow the parametric model proposed in~\cite{Wang_2019_CVPR} that formulates the layout prediction as a multi-task prediction problem, e.g. predict the number of lanes, and the existence of, and distance to various types of intersections, crosswalks and sidewalks. Then we propose to improve the representation power of our model input. In contrast to~\cite{Wang_2019_CVPR} that replies only on single image depth and semantic predictions to obtain the top-view semantic map, we instead propose to combine the information from entire video sequences, or global information, as well as context. More specifically, we utilize Structure-from-Motion (SfM)~\cite{schonberger2016structure} and Multiple View Stereo (MVS)~\cite{schonberger2016pixelwise} to obtain dense 3D reconstruction of the road scene from the video sequences; the multiview geometric constraints encoded in such method naturally allow us to generate temporally consistent top-view map for each individual view. Moreover, we combine the objects as context cues and map them to top-view as additional information. In general, our representation is more powerful and smoothed thus enables us to boost the per-image prediction accuracy. (See Fig.~\ref{fig:teaser}).

To achieve that, we first propose a novel network structure to enforce temporal smoothness in videos. Specifically, our network consists of (i) an LSTM~\cite{hochreiter1997long} that incorporates the long-range prediction coherency and (ii) a Feature Transform Module (FTM) that explicitly aggregates information w.r.t. estimated camera motion and encourages consistency on the feature level. %(Fig.~\ref{fig:teaser}). 
By explicitly and implicitly encoding temporal smoothness constraints, our proposed network is able to improve the prediction accuracy and consistency. Apart from incorporating temporal coherency in videos, we further propose to exploit context cues in scene attribute prediction in the top-view. More specifically, such cues are represented and obtained with 3D object detection~\cite{li2019gs3d,li2019stereo} and provide useful priors and constraints for layout estimation in the top-view. For instance, by looking at only the green rectangles in the "top-view representation" in Fig.~\ref{fig:teaser}, one can obtain a rough estimate of the drivable areas.

%describe the model input
%As for our model input, we propose incorporate object information, which can be obtained by applying existing 3D object localization methods~\cite{li2019stereo,li2019gs3d} on each frame, as context cues. 
The above mentioned proposals are applicable for both offline and online scene understanding in videos. When the online scenario is not required, we can further improve our model by leveraging even more powerful temporal cues from future frames. Applications like forensic analysis of traffic scenes and driver behavior studies using commodity cameras are examples where road layout estimation is required while the entire videos can be available. For such cases, we further propose to combine information obtained locally from individual frames with that obtained globally from entire video sequences. Specifically, we utilize structure from motion (SfM) \cite{schonberger2016structure} and multiple view stereo (MVS) \cite{schonberger2016pixelwise} to obtain a dense 3D reconstruction of the road scene from the video sequence. The multiview geometric constraints encoded in such methods naturally aggregate the temporal information from multiple frames, thus permitting a more coherent scene representation as compared to individual views.
% we propose to combine information obtained locally with individual frame with that globally from entire video sequences. Furthermore, we explicitly incorporate context cues, or object information, in our input. Specifically, we utilize Structure-from-Motion (SfM)~\cite{schonberger2016structure} and Multiple View Stereo (MVS)~\cite{schonberger2016pixelwise} to obtain dense 3D reconstruction of the road scene from the video sequences; the multiview geometric constraints encoded in such method naturally allow us to generate temporally consistent input. We further include object information, which can be obtained by applying existing 3D object localization methods~\cite{??} on each frame, as context cues. 
This allows us to build the model input that is of better representation power and smoother, which boosts the prediction accuracy as well as coherence (see Fig.~\ref{fig:teaser}).
%At test time, we convert a sequences of perspective RGB images into a bunch of semantic top-view representations that considers both individual, global and context information in videos, and predict our scene model's parameters coherently. 

We conduct experiments to validate our ideas on two public driving data sets, KITTI~\cite{sam:Geiger13a} and NuScenes~\cite{sam:NuScenes18a} (Sec.~\ref{sec:exps}).  Our results demonstrate the effectiveness of the global and context cues in terms of prediction accuracy, and the importance of the LSTM as well as FTM for consistent outputs.
To summarize, our key contributions are:
%
\begin{itemize}
\item A novel neural network that includes (i) an LSTM that implicitly enforces prediction coherency in videos and (ii) a Feature Transform Module that explicitly encodes the feature level consistency w.r.t. camera motion.
\item An input representation that considers information obtained (i) locally from individual frames, (ii) globally from entire video sequence and (iii) from contextual cues.
\item Experimental evaluation that outperforms state-of-the-art on public datasets by a large margin.
\end{itemize}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../param_bev"
%%% End:


==> Understanding Road Layout from Videos as a Whole (1)/sections/method.tex <==
\section{Our Framework}
\label{sec:method}
%The goal of this work is to make temporally consistent while semantically and geometrically accurate predictions on interpretable attributes of the layout of complex road scenes from video sequences. We follow the model proposed in~\cite{Wang_2019_CVPR} and briefly introduce the parameterized scene model that describes attributes like the topology of the road in Sec.~\ref{sec:scene_model}. Then we describe our first contribution in Sec.~\ref{sec:train_infer_scene_model}, where we propose a novel neural network that consists of two important components, a Feature Transform Module (FTM) (Sec.~\ref{sec:model_STM}) in top view that explicitly warps and aggregates features w.r.t. camera motion and a LSTM (Sec.~\ref{sec:model_LSTM}) that implicitly enforces temporal smoothness with aggregated features. Later, we introduce our second contribution in Sec.\ref{sec:bev_maps}. Specifically, we describe how we incorporate context information such as traffic participants in general setting and leverage global information from entire video sequence in offline scenarios.

We briefly introduce the parameterized scene model in Sec.~\ref{sec:scene_model}. Then we describe our proposed LSTM with FTM in Sec.~\ref{sec:train_infer_scene_model}, followed by the utlization of context information and global information in Sec.~\ref{sec:bev_maps}. An overview of our framework is shown in Fig.~\ref{fig:framework_overview}.

% Then we describe our first contribution in Sec.~\ref{sec:bev_maps}. Specifically, we introduce how to obtain per-frame based top-view semantic map as input for our model. This top-view map incorporates local information that comes from individual semantic and depth prediction, global information obtained with dense 3D reconstruction from COLMAP~\cite{schonberger2016structure,schonberger2016pixelwise} on the entire video sequences, and context information such as traffic participants (See Sec.\ref{sec:bev_maps}). After obtaining these top-view maps, we then introduce our second contribution in Sec.~\ref{sec:train_infer_scene_model}, where we propose a novel deep learning framework that consists of two important components, a Spatial Transform Module (STM) (Sec.~\ref{sec:model_STM}) in top view that explicitly warps and aggregates features w.r.t. camera motion and a LSTM (Sec.~\ref{sec:model_LSTM}) that implicitly enforces temporal smoothness with aggregated features in top-view.
% \begin{figure}\centering
%   \includegraphics[width=0.5\textwidth]{figures/model_example.png}
%   \vspace{-0.65cm}
%   \caption{Overview of our network. (\bing{FIXME:symbol very blurred}) }
%   \label{fig:model_overview}
% \end{figure}

\subsection{Scene Representation}
\label{sec:scene_model}
Given a monocular video sequence capturing a road in the perspective view, our goal is to obtain a coherent yet accurate road layout estimation in the top-view for each frame. To describe the top-view layout, we follow the parametric representation of~\cite{Wang_2019_CVPR}, which consists of three different types of scene attributes/variables, including $\saBinNum = 14$ binary variables $\saBin$, $\saMcNum = 2$ multi-class variables $\saMc$ and $\saRegNum = 22$ continuous variables $\saReg$.
%The camera is assumed at the bottom center of the predicted top-view~\footnote{We refer the readers to supplementary material for more details.}. See Fig.~\ref{fig:teaser} for example predicted results.
These parameters can represent a large variety of road scene layouts~\footnote{We refer to our supplementary material and~\cite{Wang_2019_CVPR} for more details.}. See Fig.~\ref{fig:teaser} for examples of predicted results.
Denoting the scene model parameters $\sa=\{\saBin,\saMc,\saReg\}$, we aim to predict $\sa^t$, the scene parameters of the $t$-th frame, coherently and accurately for all $t\in\{1,\dots,T\}$, where $T$ is the number of frames in a video. However, instead of making predictions from single image, we propose to augment the underlying feature representation and aggregate temporal information from videos for more temporally consistent and robust predictions.
%Following \cite{Wang_2019_CVPR}, the scene is described in a top-view representation with a parametric model consisting of three different types of scene attributes/variables, including $\saBinNum = 14$ binary variables $\saBin$, $\saMcNum = 2$ multi-class variables $\saMc$ and $\saRegNum = 22$ continuous variables $\saReg$. The camera is assumed at the bottom center of the predicted top-view. See Fig.~\ref{fig:teaser} for example predicted results. Note that in this paper, we apply exactly the same scene model as in \cite{Wang_2019_CVPR} and we refer the readers to~\cite{Wang_2019_CVPR} for more details for the scene model.  However, instead of making prediction from single image, we propose to augment the underlying feature representation and aggregate temporal information from videos for more temporally consistent and robust predictions. Specifically, denoting the scene model parameter $\sa=\{\saBin,\saMc,\saReg\}$, we aim to predict $\sa^t$, or the scene parameters of the $t$-th frame, coherently and accurately for all $t\in\{1,\dots,T\}$, where $T$ is the number of frames in a video. 

%Note that in this paper, instead of proposing a novel scene representation model, we specifically focus on road layout estimation in videos, e.g. boost the performance in terms of semantic and geometric accuracy as well as temporal coherency given video sequences as input.

\subsection{Our LSTM-based Model}
\label{sec:train_infer_scene_model}
% Denoting the semantic top-view $bevinit$ from a single image as $\bevmap$, and $\bevmap^t$ is the $bevinit$ at time step $t$, then the overall model is defined as the following:
In order to exploit long-term temporal information, we propose to utilize LSTM for road layout prediction. In addition, we propose a Feture Transform Module (FTM) to more explicitly aggregate temporal information. We will discuss more details below.

We denote the representation of the road scene at a certain view as $\bevmap \in \realspace^{H \times W \times C}$, and hence $\bevmap^t$ at the $t$-th frame in a video. Here, $\bevmap$ can be regarded as any generic representation such as RGB perspective image or top-view image of the road; our proposed novel top-view representation will be discussed shortly in Sec.~\ref{sec:bev_maps}.
Given $\bevmap^t$, our overall model is defined as following:
\vspace{-0.1cm}
\begin{equation}
\begin{split}
    %\bm{y}^t = \nnFull_{com}(\nnFeat_{i}(\bevmap^t),\nnFeat_{ft}(\nnFeat_{i}(\bevmap^{t-1}))), \\
    %\sa^t = \nnAttr(\nnFeat_{lstm}( \nnFeat_{j}(\bm{y}^t))),
    % What is '\bm{}'? It throws an error. Did you want to make it bold?
    y^t = \nnFull_{com}(\nnFeat_{i}(\bevmap^t),\nnFeat_{ft}(\nnFeat_{i}(\bevmap^{t-1}))), \\
    \sa^t = \nnAttr(\nnFeat_{lstm}( \nnFeat_{j}(y^t))),
\end{split}
\label{eq:total_NN}
\end{equation}
\vspace{-0.1cm}

\noindent where $\nnAttr$, $\nnFeat_{*}$ and $\nnFull_{*}$ are neural networks, with weights %$\nnAttrWgts$
$\gamma_h$, 
%$\nnFeatWgts_{*}$ and $\nnFullWgts_{*}$ 
$\gamma_{g_*}$ and $\gamma_{f_*}$
respectively, that we want to train.
%$\bm{y}^t$ is the auxiliary intermediate feature representation.
$y^t$ is the auxiliary intermediate feature representation.
Our network structure is illustrated in Fig.~\ref{fig:model_overview}.
The architecture of $\nnFeat_i$ is a shallow (one-layer) convolutional neural network (CNN) and $\nnFeat_j$ is a deeper (seven-layer) network. We firstly pass the individual input $\bevmap^t$ to $\nnFeat_i$ and receive feature $\nnFeat_i(\bevmap^t)$. Then this feature is combined with $\nnFeat_{ft}(\nnFeat_i(\bevmap^{t-1}))$, which is obtained by feeding $\nnFeat_i(\bevmap^{t-1})$, the feature obtained from previous frame, to FTM $\nnFeat_{ft}$, and feed to $\nnFeat_j$. The output of $\nnFeat_j$ is a 1-dimensional feature vector (for each frame) that is further fed into our LSTM module $\nnFeat_{lstm}$. $\nnFeat_{lstm}$ then outputs features that implicitly encode information from previous frame by incorporating hidden states from $\bevmap^{t-1}$ and send to $\nnAttr$.
Then, the function $\nnAttr$ is defined as a multi-layer perceptron (MLP) predicting the scene attributes $\sa^t$ with features obtained from LSTM module.
Specifically, $\nnAttr$ is implemented as a multi-task network with three separate predictions for each of the parameter groups of the scene model~\footnote{In experiments, we also tried both bi-directional LSTM~\cite{schuster1997bidirectional} and ConvLSTM~\cite{xingjian2015convolutional}. We did not observe significant improvements over traditional LSTM.}.

\subsubsection{Feature transform module}
\label{sec:model_STM}

Assuming that after $\nnFeat_i$, we are able to extract a feature map $\mathbf{F} = \nnFeat_i(\bevmap) \in \realspace^{h_f \times w_f \times c_f}$, where $h_f$, $w_f$, and $c_f$ denote the height, width and feature dimension. We would like the network to learn more robust feature representations by encouraging temporal consistency. To this end, we propose to aggregate the features that correspond to the same location in the scene from the nearby frames, and feed the composited features into the later prediction layers. Intuitively, we would like the network to make use of the features at the same point but from different views for more robust prediction, as well as encourage more temporally consistent feature learning.
%Our intuition behind is that, in such a way, the network would attempt to reach consensus on the feature representations that are supposed to be, in order to facilitate the final prediction with high confidence. 

%In the following, we propose a Feature Transform Module (FTM) that warps the feature in top-view and effectively aggregate information over time. 
%Such module is able to explicitly encourage temporal smoothness in predictions by enforcing feature-level consistency over frames. 


\begin{figure}[t]
	\setlength{\belowcaptionskip}{-0.35cm}
    \begin{center}
        \includegraphics[width=1.8\linewidth, trim = 0mm 40mm 25mm 100mm, clip]{figures/model_example.pdf}
    \end{center}
    \vspace{-0.75cm}
    \caption{Overview of our network.}
    \label{fig:model_overview}
\end{figure}

\noindent \textbf{Feature correspondence:}
%Although road layout is static, our camera is moving; therefore, the feature $\mathbf{F}^t$ obtained at time step $t$ and $\mathbf{F}^{t-1}$ are generally different at the same location. 
In order to aggregate the features corresponding to the same spatial location, we need to find a correspondence between two feature maps in neighbouring frames.
One obvious way to achieve this is by computing optical flow~\cite{sun2010secrets} between neighbouring perspective images and transforming the correspondence w.r.t. the flow field on the feature map. We later
% However, we shall 
show in Sec.~\ref{sec:input_ind_and_colmap} that such computation can be obviated here as we have the camera poses and 3D reconstruction of the road built from the video.

\noindent \textbf{Feature transformation:}
%\sam{The order of concepts introduced seems sub-optimal to me: Feature transformation requires the flow field S, which is used in the formula but then only later discussed in Feature correspondence, which again refers to a later section. Shouldn't the order rather be: Get the correspondence, transform the features and compose the features.} \bing{Maybe the easiest way to fix is to give an overall picture of sections in the begining?}
%Let us assume now that we have 
Given the correspondence between feature maps, we can warp~\cite{vu2018memory,zhu2017flow} the feature map at time step $t-1$ to the current time step $t$, denoted as: 
\begin{equation} 
    \nnFeat_{ft}(\mathbf{F}^{t-1}) = \phi(\mathbf{F}^{t-1},\ S^{t-1}(\bevmap^{t},\bevmap^{t-1}))
\label{eq:STM}
\end{equation} 
where $\phi(*)$ is the bilinear sampling function~\cite{sam:Jaderberg15a} and $S^{t-1}(\bevmap^{t},\bevmap^{t-1}) \in \realspace^{h_f \times w_f \times 2}$ is a displacement (or flow) field between frames $t$ and $t$-1.

\noindent \textbf{Feature composition:}
One can choose various ways to aggregate the feature map $\nnFeat_{ft}(\mathbf{F}^{t-1})$ and $\mathbf{F}^{t}$. Here, we adopt the following simple weighted summation of the two, 
\begin{equation}
    \nnFull_{com}(\mathbf{F}^t,\nnFeat_{ft}(\mathbf{F}^{t-1})) = \alpha \cdot \mathbf{F}^t +(1-\alpha)\cdot \nnFeat_{ft}(\mathbf{F}^{t-1}),
\end{equation}
where $\alpha$ can either be a scalar, e.g. $\alpha=\frac{1}{2}$, or a matrix, $\alpha \in \realspace^{h_f \times w_f}$. Note that in both cases, $\alpha$ can be automatically learned together with the rest of the network without any additional supervision. For special cases where $t = 1$, we simply assume $\nnFeat_{st}(\mathbf{F}^{t-1})$ equals to $\mathbf{F}^t$. It's simple but it works well in practice, see supp for more discussion.
%Despite its simplicity, the summation also has a few other advantages (see supplementary material for more discussion). \sam{Either provide one explicit advantage and refer to supp for more or just say: It's simple but it works well in practice, see supp for more discussion.} Indeed, empirically we find it to work well in general. 

\noindent \textbf{Discussion:} Note that we can easily extend our model by aggregating features from frames that are further away or even from future frames in offline settings. Also, FTM can be extended for multiple feature maps at different scales, which can potentially further improve the performance.

\iffalse
Intuitively, if one can find the dense correspondences between feature maps from consecutive frames, it is possible to aggregate information among frames thus to encourage the feature level consistency. To this end, we propose to utilize FTM to warp features according to scene dynamics. Specifically, we have:
\begin{equation} 
    \nnFull_{ft}(\mathbf{F}^{t-1})=\nnFeat_{st}(\nnFeat_{i}(\bevmap^{t-1}))=\phi(\mathbf{F}^{t-1},\ S^{t-1}{(\bevmap^{t},\bevmap^{t-1})
\label{eq:STM}
\end{equation} 
where $\phi(*)$ is the bilinear sampling function and $S^{t-1}({\bevmap^{t},\bevmap^{t-1}) \in \realspace^{h_f \times w_f \times 2}$ is a displacement (or flow) field between frames $t$ and $t-1$. Although one familiar way to obtain such displacement is by computing optical flow between two images, such computation can be obviated if we can obtain accurate camera poses (more details will follow in Sec.~\ref{sec:input_ind_and_colmap}). %Note that our $bevinit$ is directly cropped from the fitted road plane according to camera poses (see Fig.~\ref{fig:bevfromcolmap}(c)\&(d)), this allows us to readily have the location of each pixel in the next $bevinit$ by a simple transformation. 
%Although one familiar way to obtain such displacement is simply computing optical flow between two $bevinit$ images, such computation can be obviated in our method. Note that our $bevinit$ is directly cropped from the fitted road plane according to camera poses (see Fig.~\ref{fig:bevfromcolmap}(c)\&(d)), this allows us to readily have the location of each pixel in the next $bevinit$ by a simple transformation.
Once we obtain the features transformed from time step $t-1$ to current time step t, or $\nnFull_{st}(\mathbf{F}^{t-1})$, our next step is to aggregate the information from current time step $t$ with the transformed features. Specifically, we define our combination function as:
\begin{equation}
    \nnFull_{com}(\mathbf{F}^t,\nnFull_{st}(\mathbf{F}^{t-1})) = \alpha \cdot \mathbf{F}^t +(1-\alpha)\cdot \nnFull_{ft}(\mathbf{F}^{t-1})
\end{equation}
Where $\alpha$ can either be a scalar, e.g. $\alpha=\frac{1}{2}$, or a matrix, $\alpha \in \realspace^{h_f \times w_f}$. Note that in both cases, $\alpha$ can be learned automatically learned together with the rest of the network without any additional supervision. For special cases where $t = 1$, we simply assume $\nnFull_{st}(\mathbf{F}^{t-1})$ equals to $\mathbf{F}^t$. Note we can easily extend our model by aggregating features from frames that are further away or even from future frames in offline settings. Also, FTM can be extended for multiple feature maps at different scales, which can potentially further improve the performance.
\fi

%\subsubsection{LSTM}
%\label{sec:model_LSTM}
%While the FTM aims to enforce the consistency in feature level in videos, we also propose LSTM module that integrates temporal coherency implicitly. A typical LSTM unit contains an input gate, which determines the extent to which the input is supposed to update the memory cell at current time step, a forget gate that determines the effectiveness of the previous state of the memory cell from time step $t-1$ on its current time step $t$, an output gate that governs the amount of information output from the memory cell, and an output state, together with an internal memory cell state. In our experiment, we denote the output of LSTM module as $\nnFeat_{lstm}(*)$, where $*$ denotes the input. At time step $t$, our LSTM receives the input from $\nnFeat_{j}(\nnFull_{com}(\mathbf{F}^t,\nnFull_{st}(\mathbf{F}^{t-1})))$ as well as the hidden states from $t-1$. And the output is fed to $\nnAttr$ for final prediction task. Note that we omit the hidden states in all our equations for clarity. In experiments, we tried both bi-directional LSTM~\cite{schuster1997bidirectional} and ConvLSTM~\cite{xingjian2015convolutional}. We did not observe significant improvements with these two variants of traditional LSTM. 

\subsubsection{Loss functions on scene attribute annotation:}
Given the annotated data sets $\dsReal$ that consist of $\dsRealSize$ videos, we define our overall loss function $\lossSupReal$ as:
%
\vspace{-0.2cm}
$$\sum_{i,t}^{\dsRealSize,T} \lossBCE(\saBinRealIdx^{t}, \hat{\Theta}^t_{b,i})  + \lossCE(\saMcRealIdx^t, \hat{\Theta}^t_{m,i})+ \lossEllOne(\saRegRealIdx^t, \hat{\Theta}^t_{c,i}), $$
\vspace{-0.4cm}

%\begin{equation}
%\begin{split}
%    \sum_{i,t}^{\dsRealSize,T} & \lossBCE(\saBinRealIdx^{t}, \hat{\saBinRealIdx}^t)  + \lossCE(\saMcRealIdx^t, \hat{\saMcRealIdx}^t)+ %\lossEllOne(\saRegRealIdx^t, \hat{\saRegRealIdx}^t) \;,
%\end{split}
%\label{eq:full_loss}
%\end{equation}
\noindent where CE denotes cross-entropy and BCE represents binary cross-entropy. We further denote the ground-truth layout parameters of the $t$-th frame in the $i$-th video sequence in the data set as $\hat{\Theta}^t_{*,i}$. Note that we discretize continuous variables for the regression task -- each variable is discretized into $\numSaRegBins$=100 bins by convolving a Dirac delta function centered at $\saReg$ with a Gaussian of fixed variance~\cite{Wang_2019_CVPR}. %In all our experiments, $\numSaRegBins$ is set to 100.

\subsection{Model Input}
\label{sec:bev_maps}
As suggested by~\cite{Wang_2019_CVPR}, the form of our model input $\bevmap$ has a large impact on our model. Although a perspective RGB image is a natural representation of $\bevmap$, it does not work well in top-view layout estimations. Instead,~\cite{Wang_2019_CVPR} proposes to convert each single perspective image to semantic top-view with pixel-level depth and semantic segmentation. In our case, since we are working on videos, there are more aspects that can be explored, like long-term temporal smoothness. In this section, we propose to exploit both context and global information in videos to improve the representation of $\bevmap$.
%Given a scene layout representation as described in Sec.~\ref{sec:scene_model} and assuming that we already have data sets where paired images and ground-truth annotations are available, our next step is to design a model that takes a video sequence as input and outputs accurate while consistent per-frame predictions. To this end, we propose to both improve the representation power of model input as well as the model prediction power. The following section describes in detail how we improve the model input.


\paragraph{Local information: single frame}
Following \cite{Wang_2019_CVPR}, given a single perspective image, together with its semantic segmentation, CNN-predicted dense depth, and camera intrinsics, we could obtain a top-view image of the road by (1) back-projecting all the road pixels into a 3D point cloud and (2) projecting all the 3D points onto the x-y plane.
%we can obtain its corresponding per-pixel semantic segmentation~\cite{sam:RotaBulo18a,sam:Chen18a,sam:Zhao17a}  as well as dense depth map~\cite{sam:Godard17a,sam:Laina16a,sam:Xu18a}. Combined with the intrinsic camera parameters, we can further map each coordinate of the perspective view into the 3D space. Specifically, we drop the z-coordinate (height axis) for each 3D point and assign x and y coordinates to the closest integer.%
%as follows:
%\begin{equation}
%    X_i = \frac{x_i - P}{f} * d_i
%\end{equation}
%Where the $P$, $f$, $x_i$ and $d_i$ are the pinhole, focal length, x location (\bing{FIXME: is $x_i$ only the $x$ of pixel $i$ or the full coordinate $(x,y)$ of pixel $i$? If the formal is the case, we should mention $Y_i = \frac{y_i - P}{f} * d_i$ somewhere }) of pixel $i$ as well as its depth value in perspective image, respectively.  $X_i$ and $d_i$ is the real distance from camera to $i$-th pixel in in top-view. (\bing{FIXME: real distance? $X_i$ is the coordinate in bevinit, and $d_i$ has been defined above}) 
%Depending on the scale, we can map each pixel to some geometrically meaningful top-view space. 
We use this mapping to transfer the semantic class probability distribution of each pixel from perspective- into top-view. We call it $bev$ and denote it as $\bevmap \in \realspace^{\bevmapH \times \bevmapW \times \bevmapC}$, where $\bevmapC$ is the number of semantic classes. %In~\cite{Wang_2019_CVPR}, they set $\bevmapC=4$ and present four background classes, e.g. road, lane boundary, cross-walk and side-road. In this paper, we use 
$\bevmapH= 128$ and $\bevmapW= 64$ pixels, which relates to 60×30 meters in the point cloud. See Fig.~\ref{fig:bevinit-examples} for some examples of the $bev$ map obtained with single images. %As can be viewed in these examples, there are clearly some artifacts with these top-view images, e.g. the V-shape in the bottom and the missing details where pixels are far away. This is in essence due to the inherent limitation of single-view 3D reconstruction in terms of the resolution for the far scenes.

\subsubsection{Context information}
\label{sec:context}
Considering that incorporating context cues proves to be very beneficial in many scene understanding tasks, unlike \cite{Wang_2019_CVPR} that only includes $C=4$ classes (i.e. road, sidewalk, lane, crosswalk), we propose to further encode an object class in $\bevmap$ (so $C=5$). Specifically, we observe that traffic participants, i.e. vehicles like cars, are commonly present in driving scenarios and can be very useful for layout estimation, e.g. side-faced cars are informative in terms of predicting the existence of or even the distance to side-road. 
%For instance, if we observe some side-faced cars are of $x$ meters away, it is very likely that it is where the side-road lies. Similarly, if cars are driving along the main road, they also provide us information about the coverage of main road.
%To this end, we introduce one object layer in $bevinit$. In our paper $\bevmapC=5$ while $\bevmap=4$ in~\cite{Wang_2019_CVPR}. %Assuming that we are able to detect/segment cars in video sequences, we then can map them to top-view space. 
One naive way to incorporate context cues
% perform it \sam{Perform what?} 
is to follow what is done for other classes to directly map the pixel-level probabilities of objects to top-view. However, we observe that this naive method would lead to diffused representations\footnote{This is mainly due to the small size of the objects, making it less robust to semantic and depth prediction noise when mapping to top-view.} (See Fig.~\ref{fig:obj_example} for examples) and can be very noisy. Instead, we propose to utilize the bounding box representation. Specifically, we apply existing 3D object detectors~\cite{li2019gs3d,li2019stereo} on our videos and map the detection results into top-view. In order to reduce the impact of angle predictions, we further propose to categorize angles into two types, frontal-faced and side-faced. As long as the predicted yaw angle is within $[-\frac{\pi}{4},\frac{\pi}{4}]$ or $[\frac{3\pi}{4},\frac{5\pi}{4}]$ w.r.t. camera $z$-axis (forward direction), we assume this predicted object is frontal-faced. Otherwise, it is side-faced (Fig.~\ref{fig:obj_example}).
% for examples). 

\begin{figure}
    \setlength{\belowcaptionskip}{-0.35cm}
	\begin{center}
	    \vspace{-0.35cm}
		\includegraphics[width=0.4\textwidth, trim = 8mm 65mm 85mm 0mm, clip]{figures/qualit_res/obj_example.pdf} \\
	\end{center}	
	\vspace{-0.55cm}
  \caption{Two examples comparing the box representation and the point cloud representation of the cars. We can observe four frontal-faced cars in both (a) and (b) and one side-faced car in (b). %We visualize the heat map for corresponding layers in $bevinit$. 
  %The brighter the color is, the higher the probability that pixel is for the corresponding class. The first row demonstrates how we propose to represent objects, or context cues. The second row gives examples on how context cues look for the same four images if we reply only on pixel-level segmentation and depth maps. The last row visualizes the layer for road, lane, crosswalk, sidewalk and car from left to right.\bing{add title like "road" below each image, shorten the caption. Also make the figure smaller.}}\
  }
  \label{fig:obj_example}
\end{figure}
\vspace{-0.35cm}


\subsubsection{Global information from video sequence}
\label{sec:input_ind_and_colmap}

As can be viewed in individual frame examples in Fig.~\ref{fig:bevinit-examples}, there are clearly some artifacts with $bev$, e.g. the V-shape in the bottom and the missing details where pixels are far away. This is in essence due to the inherent limitation of single-view 3D reconstruction in terms of the resolution for far away points in the scene.

\noindent \textbf{Top-view map from COLMAP:} When the input is an entire video sequence, we are able to address the above mentioned artifacts in an individual frame by generating a more complete 3D reconstruction as well as the subsequent $bev$. Specifically, we make use of state-of-the-art SfM and MVS algorithms from COLMAP~\cite{schonberger2016structure,schonberger2016pixelwise}, as well as the semantic segmentation in 2D image, in order to generate the top-view map (denoted as $bev$-$col$) from a video. The pipeline is illustrated in Fig.~\ref{fig:bevfromcolmap}. We first perform 3D semantic segmentation on the dense point cloud returned from COLAMP. We project each 3D point into the images as per the visibility map to obtain the semantic candidates from the 2D semantic segmentation; a simple winner-take-all strategy is applied to determine the final semantic label for each point (Fig.~\ref{fig:bevfromcolmap}(b)). The 3D semantic segmentation allows us to extract the 3D points for the road part, to which we fit a 2D plane via RANSAC (Fig.~\ref{fig:bevfromcolmap}(c)). 
%We make use of a few heuristics to make the road plane %recovery more robust, such as all the cameras being at %roughly the same height above the road plane, camera %viewing directions almost being parallel to the road %surface etc.
Finally, we can generate the $bev$-$col$ by cropping a rectangular box on the 2D road plane according to the camera pose and our pre-defined top-view image size and resolution; the 3D points on the plane are converted into the pixels in the image (Fig.~\ref{fig:bevfromcolmap}(d)). After obtaining the global plane parameters, we utilize the camera pose to transform the global plane parameters to the local parameters with respect to the camera. Note that in a well-calibrated case where the global plane can be the same as local plane, the global lane estimation process can be skipped.
%~\buyu{After obtaining the global plane parameters, we utilize the camera pose to transform the global plane parameters to the local parameters with respect to the camera. Due to the high accuracy of COLMAP, this approach is sufficient to align the local and global planes. Note that in a well-calibrated case where the global plane can be the same as local plane, the global lane estimation process can be skipped}. \bing{But, here, we know the local plane, and we say the global plane can be aligned with local plane well, isn't this is well-calibrated case?} 
See Fig.~\ref{fig:bevinit-examples} for two more examples. Here, one can see that the dense correspondence between two $bev$-$col$ can be trivially obtained given the known position and orientation of each $bev$-$col$ in the 2D road plane. Such mapping is transferred to the correspondence on the feature map and fed into FTM (Sec.~\ref{sec:model_STM}). Here, we do not handle the mapping of dynamic objects, but find FTM to still work well~\footnote{Having access to GT masks for dynamic objects may help to improve performance, but in their absence, even our current handling of dynamic objects yields promising results.}. Finally, we also note that the absolute scale of the 3D reconstruction here can be retrieved from either GPS or camera-ground height in driving scenes.

\begin{figure}\centering
\setlength{\belowcaptionskip}{-0.35cm}
\vspace{-0.35cm}
  \includegraphics[width=0.4\textwidth, trim = 10mm 0mm 120mm 0mm, clip]{figures/BEVfromColmap.pdf}
  \vspace{-0.6cm}
  \caption{An example illustration of generating semantic $bev$-$col$. (a)(b) 3D scene reconstruction and semantic segmentation. (c) road extraction and plane fitting. (d) $bev$-$col$ for the view (e). }
  \label{fig:bevfromcolmap}
\end{figure}

\begin{figure}
    \setlength{\belowcaptionskip}{-0.35cm}
	\centering
	   \includegraphics[width=0.4\textwidth, trim = 0mm 73mm 140mm 0mm, clip]{figures/elwms_colmap.pdf}
		%\includegraphics[width=0.45\textwidth]{figures/qualit_res/elwms_example.png} \\
		%\includegraphics[width=0.45\textwidth]{figures/qualit_res/colmap_example.png}\\
		% \includegraphics[width=0.45\textwidth]{figures/qualit_res/combined_example.png} \\
	\vspace{-0.35cm}
  \caption{Two examples of $bev$ and $bev$-$col$ on the background classes obtained from individual frame and COLMAP. Red circles highlight the differences.}
  %As can be viewed in this figure, results obtained with local cues only focus more on near-by areas while those with global information concentrate on texture regions. % They can be mutual informative and combining local and global together provides us a better $bevinit$ than either. %(\bing{TODO: We need to explain more why the individual depth prediction version from [33] is still kept in our input even though we have used the COLMAP multi-frame version. People may naturally think that the individual frame $bevinit$ is redundant if we have a more complete one from multiview. We could say that the geometry based 3D reconstruction might be inaccurate or incomplete in some challenging cases like texture-less region, and in such case the data-driven CNN-predicted depth could be more reliable and contribute more towards the layout prediction.})
  %\bing{shorten the caption.}}}
  \label{fig:bevinit-examples}
\end{figure}

\noindent \textbf{Discussion:} Note that in our case, rather than presenting what can be actually seen in the current frame, our $bev$-$col$ obtained with COLMAP models what really exists. For instance, a sideroad that is far away or occluded can hardly be noticed in $bev$ generated from an individual frame only due to the lack of observations in perspective view. In contrast, $bev$-$col$ generated with global information is able to recover the sideroad properly as long as we have observations in this video (see comparison in Fig.~\ref{fig:bevinit-examples}(a)).   

% Note that in this case, our $bevinit$ does not represent what can be actually seen in current frame. Instead, we aim to model that really exists w.r.t. current frame. For instance, a crosswalk can only consume a small of proportion of pixels in perspective image if it is far away from camera. In this case, our individual frame method only map very few crosswalk into top-view maps and potentially would introduce errors/problems for model prediction. However, when we take the entire video sequence into consideration, we are aware of the existence as well as the number of pixels that belongs to this crosswalk. Even the crosswalk is far away, we can model it with a more clear while informative way. Some examples of our video-based top-view maps generation results can be found in Fig.~\ref{fig:bevinit-examples} (second row).

\noindent \textbf{Final input:} Our final input incorporates local information from individual frame, global information from videos and object-level context information. Note that local and global cues can be mutually informative, e.g. geometry based 3D reconstruction might be inaccurate or incomplete in some challenging cases like texture-less regions, but in such cases the top-view information from CNN-predicted depth could be more informative towards the layout prediction (See comparison in Fig.~\ref{fig:bevinit-examples}(b)). In summary, our proposed top-view semantic map $bev$-$final$ is in $\realspace^{\bevmapH \times \bevmapW \times \bevmapC}$, where $\bevmapC=5$ and the layers represents four background classes and car; We overlay $bev\text{-}col$ on top of $bev$ to fuse them together. Specifically, for a binary mask $B$ with $B_{i,j}{=}1$ if $bev\text{-}col_{i,j}{\neq}0$, we have $bev \text{-}final=bev\text{-}col{\odot} B+bev{\odot}(1{-}B)$, where $\odot$ indicates element-wise product. See an example visualization of each layer in Fig.~\ref{fig:bevinit-context-example}. 

\begin{figure}
    \setlength{\belowcaptionskip}{-0.35cm}
	\centering
	% \vspace{-0.35cm}
	\begin{tabular}{c}
		\includegraphics[width=0.45\textwidth, trim = 0mm 65mm 80mm 5mm, clip]{figures/qualit_res/layers_res.pdf} \\
	\end{tabular}
	\vspace{-0.35cm}
  \caption{An example visualizing the layers in our $bev$-$final$. %The brighter the color is, the higher the probability that pixel belongs to the corresponding class.
  %\bing{Buyu, point me to the RGB image so I can add it on the left}. %We visualize the heat map for corresponding layers in $bevinit$. 
  %The brighter the color is, the higher the probability that pixel is for the corresponding class. The first row demonstrates how we propose to represent objects, or context cues. The second row gives examples on how context cues look for the same four images if we reply only on pixel-level segmentation and depth maps. The last row visualizes the layer for road, lane, crosswalk, sidewalk and car from left to right.\bing{add title like "road" below each image, shorten the caption. Also make the figure smaller.}}
  }
  \label{fig:bevinit-context-example}
\end{figure}

% \subsection{Training and Inferring the Scene Model}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../param_bev"
%%% End:


==> Understanding Road Layout from Videos as a Whole (1)/sections/related_work.tex <==
\section{Related Work}
\label{sec:related}
Scene understanding is an important yet challenging task in computer vision, which enables us to perform applications such as robot navigation~\cite{sam:Gupta17a}, autonomous driving~\cite{sam:Geiger14a,sam:Kunze18a}, augmented reality~\cite{sam:Armeni16a} or real estate~\cite{sam:Liu15a,sam:Song18a}.

\paragraph{3D scene understanding:} 3D scene understanding 
%requires comprehensive understanding for given scenes. Among all, it 
is most frequently explored for indoor scenes~\cite{sam:Armeni16a,sam:Liu15a,sam:Song17a},  which is typically formulated as a room layout estimation problem. However, unlike the indoor scenes where strong priors, e.g. Manhattan world assumption, are available, scene understanding for outdoor scenarios is less constrained, thus can be more challenging. To this end, many non-parametric approaches have been proposed~\cite{sam:Guo12a,Tighe_2014_CVPR,sam:Tulsiani18a}, where layered representations are utilized to reason about the geometry as well as semantics in occluded areas. %Although these representations naturally reflect the relative orders, they are not able to model the absolute distance information. In contrast, 
More recent work~\cite{sam:Schulter18a,sam:Sengupta12a} propose top-view representations to provide a more detailed description for outdoor scenes in 3D. As for parametric models, Seff and Xiao~\cite{sam:Seff16a} propose a model that consists of certain road scene attributes and further utilize a neural network to directly predict them from a single perspective RGB image. However, these pre-defined attributes are not rich enough to capture various types of road layout. A more recent work~\cite{sam:Kunze18a} presents a graph-based road representation that includes lanes and lane markings, from partial segmentation of an image. However, this representation focuses on straight roads only. Similarly, an interesting model is proposed by M\'{a}ttyus~\etal~\cite{sam:Mattyus16a} to augment existing map data with richer semantics. Again, this model only handles straight roads and requires additional input from aerial images. To further handle complex road layouts with traffic participants, Geiger~\etal~\cite{sam:Geiger14a} propose to utilize multiple modalities as input, such as vehicle tracklets, vanishing points and scene flow. Recently, a richer model~\cite{Wang_2019_CVPR} is proposed to handle more complex road scenarios, e.g. multiple lanes and different types of intersections. Our work follows the parametric representation proposed in~\cite{Wang_2019_CVPR}. Unlike~\cite{Wang_2019_CVPR} that only takes local information, e.g. pixel-level depth and semantic segmentation from a single frame, we propose to explore multiple aspects in videos, e.g. global information and context cues, to obtain accurate and coherent predictions.

\vspace{-0.5cm}
\paragraph{Scene understanding in videos:} 
Apart from accuracy, scene understanding in videos further requires consistent predictions between consecutive frames. Spatio-temporal probabilistic graphical models~\cite{liu2015multiclass,Wang_2019_CVPR} are widely explored for outdoor scenes. Nowadays, recurrent neural networks (RNNs) like LSTMs~\cite{donahue2015long,hochreiter1997long,srivastava2015unsupervised} are used to propagate feature representations from still frames over time. However, LSTMs implicitly enforce the prediction consistency without the explicit knowledge of motion. To this end, more recent work~\cite{feichtenhofer2017spatiotemporal,simonyan2014two} propose to combine features extracted from both images and motion, or optical flow, to boost the representational power. Although motion is fed as additional input for networks in these above mentioned networks, it is not utilized to transform features over time to explicitly enforce the feature level consistency. Maybe~\cite{vu2018memory,zhu2017flow} are the most closest work to ours in terms of feature warping and aggregation. Specifically, ~\cite{zhu2017flow,zhu2017deep} explicitly warp feature maps~\cite{fischer2015flownet} between frames and propose to aggregate them in a more well-aligned manner. To address the fixed temporal width problem in~\cite{zhu2017flow}, more recent work~\cite{vu2018memory} introduces a feature memory that is warped from one frame to another, which enables a longer temporal horizon without looking into future frames. In contrast, we introduce a Feature Transform Module (FTM) that warps features w.r.t camera motion and aggregates them between consecutive frames. And we further propose to combine LSTM and FTM to implicitly and explicitly enforce temporal smoothness in predictions. %And LSTM takes the aggregated information and further enforce prediction coherency. 
More importantly, unlike prior methods that estimate flow in the perspective view of the scene, all our modules work in the top-view space.

\begin{figure*}[t]
 \setlength{\belowcaptionskip}{-0.35cm}
 \centering
 \vspace{-0.3cm}
  \includegraphics[width=1.0\linewidth, trim = 0mm 100mm 0mm 0mm, clip]{figures/model_example.pdf}
  \vspace{-0.65cm}
  \caption{\textbf{Overview of our proposed framework:} Given videos as input, top-view maps aggregated from local, global and context information, are fed into our FTM/LSTM network to predict the parametric road scene layout. %Our goal is to provide consistent yet accurate road layout predictions with given video sequences. We follow the work~\cite{Wang_2019_CVPR} and formulate our problem as a hybrid road attribute prediction problem. Given one video sequence, we firstly propose to map these perspective images to semantic top-view space with both local and global information. Meanwhile, we propose to incorporate context information in top-view space, which is represented by object-level cues in our paper. Then we send these top-view maps to a novel network, which consists of a FTM that is designed to explicitly aggregate information in top-view by warping features w.r.t. camera motion and a LSTM to implicitly enforce prediction smoothness.}
  }
  \label{fig:framework_overview}
\end{figure*}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../param_bev"
%%% End:


==> Understanding Road Layout from Videos as a Whole (1)/tables/ablation_single.tex <==
\begin{tabular}{l|cccc}
  \hline
              &  \multicolumn{4}{c}{KITTI~\cite{sam:Geiger13a}} \\
  \hline
  Method      &  Accu.-Bi. $\uparrow$ & Accu.-Mc. $\uparrow$ & MSE $\downarrow$ & F1.-Bi. $\uparrow$\\
  \hline
  BEV-C          & .826& .779& .175& .456  \\
  \hline
  *-denseC & .826      & .783     & .148 & .496 \\ 
  *-C-O     & .836 & .812 & .146 & .507  \\  
  \hline
  *+LSTM     & .831 & .812 & .136 & .360  \\  
  \hline  
\end{tabular}

==> Understanding Road Layout from Videos as a Whole (1)/tables/consistency_check.tex <==
% \begin{tabular}{l|cc|cc}
%   \hline
%               &  \multicolumn{2}{c|}{KITTI~\cite{sam:Geiger13a}} & \multicolumn{2}{c}{NuScenes~\cite{sam:NuScenes18a}} \\
%   \hline 
%   Method      &  seman.$\downarrow$& temp.$\downarrow$ & seman.$\downarrow$ & temp.$\downarrow$ \\ 
%   \hline
%   BEV~\cite{Wang_2019_CVPR} & 2.65& 3.99& 1.09 & 1.27\\
%   H-BEV-DA~\cite{Wang_2019_CVPR}+GM& 1.77& 1.93&  0.11 & 0.42\\                  
%   \hline
%   BEV-J-O & 1.26 & 2.78&  0.52& 1.14\\
%   \hline
%   +LSTM+FTM & 1.26 & 1.96& 0.10 & 0.51\\
% \end{tabular}

\begin{tabular}{l|cc}
  \hline
              &  \multicolumn{2}{c}{KITTI~\cite{sam:Geiger13a}} \\
  \hline 
  Method      &  seman.$\downarrow$& temp.$\downarrow$ \\ 
  \hline
  BEV~\cite{Wang_2019_CVPR} & 2.65& 3.99\\
  H-BEV-DA~\cite{Wang_2019_CVPR}+GM& 1.77& 1.93\\                  
  \hline
  BEV-J-O & 1.26 & 2.78\\
  \hline
  +LSTM+FTM & 1.26 & 1.96\\
\end{tabular}

==> Understanding Road Layout from Videos as a Whole (1)/tables/main_exp_layout.tex <==
\begingroup
\setlength{\tabcolsep}{1.8pt}
\begin{tabular}{p{3cm}|p{1.7cm}p{1.8cm}p{1cm}p{1.3cm}p{0.9cm}}
  \hline
              &  \multicolumn{5}{c}{KITTI~\cite{sam:Geiger13a}} \\
  \hline
  Method      &  Accu.-Bi. $\uparrow$ & Accu.-Mc. $\uparrow$ & MSE $\downarrow$ & F1.-Bi $\uparrow$ & IOU $\uparrow$  \\
  \hline\hline
  RGB~\cite{sam:Seff16a}          & .811& .778& .230& .176 & .327\\
  RGB~\cite{sam:Seff16a}+D        & .818  & .819  & .154&  .109 & .334\\
  BEV~\cite{Wang_2019_CVPR}      & .820& .797& .141& .324 & .345\\
  BEV~\cite{Wang_2019_CVPR}+GM  & .831& .802& .136& .344 & .357\\
  H-BEV-DA\cite{Wang_2019_CVPR}+GM  & .834 & .831 & \textbf{.134} & .435 & .404\\
  \hline
  \hline
  BEV-C          & .826& .779& .175& .456 & .317\\
  BEV-J        & .840 & .832  & .135 & .458 & \textbf{.416}\\
  BEV-J-O      & .831 & \textbf{.837}  & .142 & .494 & .388\\  
  \hline
  +LSTM        & \textbf{.845}  & .825  & \textbf{.134}  & \textbf{.537}  & .382 \\
  +LSTM+FTM      & \textbf{.842} & \textbf{.841} & \textbf{.134} & \textbf{.534} & \textbf{.405} \\    
  \hline
\end{tabular}
\endgroup

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../param_bev"
%%% End:


==> Understanding Road Layout from Videos as a Whole (1)/tables/nuscene_results.tex <==
% \begin{tabular}{l|ccccc}
%   \hline
%               & \multicolumn{5}{c}{NuScenes~\cite{sam:NuScenes18a}} \\
%   \hline
%   Method      & Accu.-Bi. $\uparrow$ &  Accu.-Mc. $\uparrow$ & MSE $\downarrow$ & F1.-Bi $\uparrow$ & IOU $\uparrow$ \\
%   \hline\hline
%   % M-BEV^*~\cite{??}      & .861      & .570      & .021 & .276 & .288 \\
%   % \hline
%   M-BEV-C          & .856    & .471      & .069 & .100 & .211\\
%   M-BEV-J        & .872      & .486      & .036 & .116 & .230\\
%   M-BEV-J-O      & .858      & .543      & .027 & .101 & .313\\  
%   \hline
%   +LSTM        &   &   &   &   &     \\
%   +LSTM+STM      &  &  &  &  & \\    
%   \hline
% \end{tabular}

\begin{tabular}{l|cccc}
  \hline
              & \multicolumn{4}{c}{NuScenes~\cite{sam:NuScenes18a}} \\
  \hline
  Method      & Accu.-Bi. $\uparrow$ &  Accu.-Mc. $\uparrow$ & MSE $\downarrow$ & IOU $\uparrow$ \\
  \hline\hline
 % ~\cite{Wang_2019_CVPR} & .855 & .626 & .033 & .450 \\
  BEV          & .846    & .485      & .073 & .217\\
  \hline
  BEV-C          & .856    & .471      & .069 & .211\\
  BEV-J        & \textbf{.872}      & .486      & .036 & .230\\
  BEV-J-O      & .858      & \textbf{.543}      & .027 & \textbf{.313}\\  
  \hline
  +LSTM        & .859 & .536  & \textbf{.023}  &  .311  \\
  +LSTM+FTM      & \textbf{.863} & \textbf{.547} & \textbf{.023} & \textbf{.328} \\    
  \hline
\end{tabular}

==> Understanding Road Layout from Videos as a Whole (1)/tables/supp_nuscenes_accuracy.tex <==
%\begin{tabular}{l|cccc}
%  \hline
%              & \multicolumn{4}{c}{NuScenes~\cite{sam:NuScenes18a}} \\
%  \hline
%  Method      & Accu.-Bi. $\uparrow$ &  Accu.-Mc. $\uparrow$ & MSE $\downarrow$ & IOU $\uparrow$ \\
%  \hline\hline
%  BEV~\cite{Wang_2019_CVPR}          & .846    & .485      & .073 & .217\\
%  H-BEV+DA~\cite{Wang_2019_CVPR}+GM & \textbf{.877} & .496 & .032 & \textbf{.326} \\
%  \hline
%  BEV-C          & .856    & .471      & .069 & .211\\
%  BEV-J        & \textbf{.872}      & .486      & .036 & .230\\
%  BEV-J-O      & .858      & \textbf{.543}      & .027 & .313\\  
%  \hline
%  +LSTM        & .859 & .536  & \textbf{.023}  &  .311  \\
%  +LSTM+FTM      & .863 & \textbf{.547} & \textbf{.023} & \textbf{.328} \\    
%  \hline
%\end{tabular}

\begin{tabular}{l|ccc}
  \hline
              & \multicolumn{3}{c}{NuScenes~\cite{sam:NuScenes18a}} \\
  \hline
  Method      & Accu.-Bi. $\uparrow$ &  Accu.-Mc. $\uparrow$ & MSE $\downarrow$ \\
  \hline\hline
  BEV~\cite{Wang_2019_CVPR}          & .846    & .485      & .073\\
  H-BEV+DA~\cite{Wang_2019_CVPR}+GM & \textbf{.877} & .496 & .032\\
  \hline
  BEV-C          & .856    & .471      & .069\\
  BEV-J        & \textbf{.872}      & .486      & .036\\
  BEV-J-O      & .858      & \textbf{.543}      & .027\\  
  \hline
  +LSTM        & .859 & .536  & \textbf{.023}\\
  +LSTM+FTM      & .863 & \textbf{.547} & \textbf{.023}\\    
  \hline
\end{tabular}

==> Understanding Road Layout from Videos as a Whole (1)/tables/supp_nuscenes_consistency.tex <==
\begin{tabular}{l|cc}
  \hline
              & \multicolumn{2}{c}{NuScenes~\cite{sam:NuScenes18a}} \\
  \hline 
  Method      &  seman.$\downarrow$& temp.$\downarrow$ \\
  \hline
  BEV~\cite{Wang_2019_CVPR} & 1.09 & 1.27\\
  H-BEV-DA~\cite{Wang_2019_CVPR}+GM&  0.07 & 0.52 \\                  
  \hline
  BEV-J-O &  0.52& 1.14\\
  \hline
  +LSTM+FTM & 0.10 & 0.51\\
\end{tabular}

==> tables/supp_nuscenes_accuracy.tex <==
%\begin{tabular}{l|cccc}
%  \hline
%              & \multicolumn{4}{c}{NuScenes~\cite{sam:NuScenes18a}} \\
%  \hline
%  Method      & Accu.-Bi. $\uparrow$ &  Accu.-Mc. $\uparrow$ & MSE $\downarrow$ & IOU $\uparrow$ \\
%  \hline\hline
%  BEV~\cite{Wang_2019_CVPR}          & .846    & .485      & .073 & .217\\
%  H-BEV+DA~\cite{Wang_2019_CVPR}+GM & \textbf{.877} & .496 & .032 & \textbf{.326} \\
%  \hline
%  BEV-C          & .856    & .471      & .069 & .211\\
%  BEV-J        & \textbf{.872}      & .486      & .036 & .230\\
%  BEV-J-O      & .858      & \textbf{.543}      & .027 & .313\\  
%  \hline
%  +LSTM        & .859 & .536  & \textbf{.023}  &  .311  \\
%  +LSTM+FTM      & .863 & \textbf{.547} & \textbf{.023} & \textbf{.328} \\    
%  \hline
%\end{tabular}

\begin{tabular}{l|ccc}
  \hline
              & \multicolumn{3}{c}{NuScenes~\cite{sam:NuScenes18a}} \\
  \hline
  Method      & Accu.-Bi. $\uparrow$ &  Accu.-Mc. $\uparrow$ & MSE $\downarrow$ \\
  \hline\hline
  BEV~\cite{Wang_2019_CVPR}          & .846    & .485      & .073\\
  H-BEV+DA~\cite{Wang_2019_CVPR}+GM & \textbf{.877} & .496 & .032\\
  \hline
  BEV-C          & .856    & .471      & .069\\
  BEV-J        & \textbf{.872}      & .486      & .036\\
  BEV-J-O      & .858      & \textbf{.543}      & .027\\  
  \hline
  +LSTM        & .859 & .536  & \textbf{.023}\\
  +LSTM+FTM      & .863 & \textbf{.547} & \textbf{.023}\\    
  \hline
\end{tabular}

==> tables/supp_nuscenes_consistency.tex <==
\begin{tabular}{l|cc}
  \hline
              & \multicolumn{2}{c}{NuScenes~\cite{sam:NuScenes18a}} \\
  \hline 
  Method      &  seman.$\downarrow$& temp.$\downarrow$ \\
  \hline
  BEV~\cite{Wang_2019_CVPR} & 1.09 & 1.27\\
  H-BEV-DA~\cite{Wang_2019_CVPR}+GM&  0.07 & 0.52 \\                  
  \hline
  BEV-J-O &  0.52& 1.14\\
  \hline
  +LSTM+FTM & 0.10 & 0.51\\
\end{tabular}
